Towards Porting Operating Systems with Program Synthesis

The end of Moore's Law has ushered in a diversity of hardware not seen in decades. Operating system (and system software) portability is accordingly becoming increasingly critical. Simultaneously, there has been tremendous progress in program synthesis. We set out to explore the feasibility of using modern program synthesis to generate the machine-dependent parts of an operating system. Our ultimate goal is to generate new ports automatically from descriptions of new machines. One of the issues involved is writing specifications, both for machine-dependent operating system functionality and for instruction set architectures. We designed two domain-specific languages: Alewife for machine-independent specifications of machine-dependent operating system functionality and Cassiopea for describing instruction set architecture semantics. Automated porting also requires an implementation. We developed a toolchain that, given an Alewife specification and a Cassiopea machine description, specializes the machine-independent specification to the target instruction set architecture and synthesizes an implementation in assembly language with a customized symbolic execution engine. Using this approach, we demonstrate successful synthesis of a total of 140 OS components from two pre-existing OSes for four real hardware platforms. We also developed several optimization methods for OS-related assembly synthesis to improve scalability. The effectiveness of our languages and ability to synthesize code for all 140 specifications is evidence of the feasibility of program synthesis for machine-dependent OS code. However, many research challenges remain; we also discuss the benefits and limitations of our synthesis-based approach to automated OS porting.

==> Makefile <==
PAPER=paper.tex
TEXFILES=\
	abstract.tex intro.tex overview.tex ale.tex casp.tex lower.tex \
	impl.tex validation.tex disc.tex rw.tex conclusion.tex

TEXFILES+=\
	tr_appendix.tex \
	./tr/notation_text.tex \
	./tr/lang_text.tex \
	./tr/check_text.tex \
	./tr/exec_text.tex \
	./tr/ale_lang_text.tex \
	./tr/ale_check_text.tex \
	./tr/ale_exec_text.tex

TEX=latex
BIBTEX=bibtex

############################################################

.SUFFIXES: .tex .dvi .ps .pdf

all: $(PAPER:.tex=.pdf)

$(PAPER:.tex=.pdf): $(TEXFILES) $(PAPER:.tex=.bib)

.tex.pdf:
	pdf$(TEX) $<
	$(BIBTEX) $(PAPER:.tex=)
	pdf$(TEX) $<
	pdf$(TEX) $<

clean:
	rm -f *~ *.dvi *.ps *.log *.aux *.bbl *.blg
	rm -f $(PAPER:.tex=.pdf)

.PHONY: clean



==> tr/commands.tex <==
%new macros for princess TRs and papers

\newcommand{\NEW}[1]{\textcolor{cyan}{#1}}
\newcommand{\NEWW}[1]{\textcolor{blue}{#1}}
\newcommand{\NNEW}[1]{\textcolor{green}{#1}}

\renewcommand{\NEW}[1]{#1}
\renewcommand{\NEWW}[1]{#1}
\renewcommand{\NNEW}[1]{#1}

\newcommand{\XXX}[1]{\textcolor{red}{#1}}
%\newcommand{\XXX}[1]{}

% because morecommands.tex needs to use \renewcommand for some things,
% because of symbol conflicts with a different (older) version of the
% same macros in ../toplas, we need to provide stub definitions here.
% XXX clean all that up and get rid of these.
\newcommand{\ensm}{\XXX{WRONG}}
\newcommand{\ttid}{\XXX{WRONG}}
\newcommand{\ttmemid}{\XXX{WRONG}}
\newcommand{\ttmemidi}{\XXX{WRONG}}
\newcommand{\bvtyp}{\XXX{WRONG}}
\newcommand{\bvaltyp}{\XXX{WRONG}}
\newcommand{\bvltyp}{\XXX{WRONG}}
\newcommand{\ttC}{\XXX{WRONG}}
\newcommand{\ttN}{\XXX{WRONG}}
\newcommand{\ttloc}{\XXX{WRONG}}
\newcommand{\ttmlen}{\XXX{WRONG}}
\newcommand{\ttbit}{\XXX{WRONG}}
\newcommand{\ttwptr}{\XXX{WRONG}}
\newcommand{\ttwvec}{\XXX{WRONG}}
\newcommand{\ttbool}{\XXX{WRONG}}
\newcommand{\ttint}{\XXX{WRONG}}
\newcommand{\ttinparen}{\XXX{WRONG}}
\newcommand{\atyp}{\XXX{WRONG}}
\newcommand{\memtyp}{\XXX{WRONG}}
\newcommand{\labeltyp}{\XXX{WRONG}}
\newcommand{\nbitmemtyp}{\XXX{WRONG}}
\newcommand{\ptrform}{\XXX{WRONG}}
\newcommand{\bnfeq}{\XXX{WRONG}}
\newcommand{\bnfor}{\XXX{WRONG}}
\newcommand{\aprimitivetyp}{\XXX{WRONG}}

\input{morecommands}




==> tr/intro.tex <==
%\documentclass[casp-main.tex]{subfiles}
 
%\begin{document}

%\include{commands}
\input{commands}

\section{Introduction}
\input{intro_text}

\section{Notation}
\input{notation_text}

%\end{document}


==> tr/intro_text.tex <==
The goal of the \aquarium project is to synthesize the machine-dependent
parts of an operating system.
This has the potential to greatly reduce the amount of work needed
to port an operating system to a new machine architecture.
It also potentially reduces the depth of knowledge needed to do that
work -- currently an OS port requires deep expert knowledge of both
the OS and the new machine architecture -- and with luck the overall
amount of time involved as well.

This document does not discuss either code synthesis or OS porting in
any detail.
It is intended as a supplement to other project publications, which
should in general be read first.
While this document includes discussions of and rationales for
language features (as well as absence of language features) these
discussions assume familiarity with the surrounding context.

The two languages described in this document are \casp\footnote{
% This really should be conditionalized on the anonymous setting... XXX
\casp is named for a jelly(fish) that features symbiotic
photosynthetic algae, which is for some reason spelled without 
the customary 'i'.
}, which is a
register-transfer-list-style machine description language used for writing
down the semantics of processor instruction sets, and \ale, which
is a specification or modeling language used for writing down
machine-independent specifications for assembly language code blocks
to be synthesized.
%(Note that \casp{} is named for a jelly(fish), whose name for some
%reason is spelled differently from the legendary queen and
%constellation.)

\casp also includes material for writing machine-dependent specifications
(this is the target for the \ale translator), a concept of mapping
modules used by the \ale translator, and a simple representation of
basic blocks in assembly language.
These are described in this document.

This document does not, however, describe any of the other languages
or file formats used in the \aquarium project or any of the \aquarium
tools.

The document is structured with six parts:
\begin{itemize}
\item The \casp language and abstract syntax (Sec. \ref{sec:lang})
\item \casp types (Section \ref{sec:check})
\item \casp semantics (Section \ref{sec:exec})
\item The \ale language and abstract syntax (Section \ref{sec:ale_lang})
\item \ale types and semantics (Section \ref{sec:ale_check})
\item \ale translation to \casp (Section \ref{sec:ale_exec})
\end{itemize}



==> usecasedescs.tex <==
\section{Complete Descriptions of Use Case Procedures}

While the details of the particular blocks in the use cases, and the
way they sequence into full procedures, are not
particularly important relative to the contributions of this paper,
they may be of interest to the reader.
In the following sections we explain them in more detail than in
\autoref{sec:usecases}.

\subsection*{\textbf{swi-handler} (SH)}

As mentioned in \autoref{sec:usecases} this is the handler for system
call traps, and it is based on the handwritten code from the
Barrelfish ARMv7 port.
We generate comparable handlers for MIPS, RISC-V, and x86\_64.
For MIPS and RISC-V these do not include logic for determining whether
a trap is a system call trap; on MIPS we also do not handle how to get
to this handler from the trap entry point (which is at a fixed
memory address).
On x86\_64 we produce the special-purpose system call handler for the
SYSCALL instruction; handlers for other traps are somewhat different.

There are 13 synthesis blocks described in \autoref{sec:usecases}, but
the grand total number of blocks is 18, one of which appears twice.

\subsubsection*{\textit{prepare}} (handwritten)

This block is here to allow setting a machine-specific assembler mode
on MIPS that is required for writing trap code.
The MIPS register usage conventions reserve one register (\$1) for use
by the assembler when expanding synthetic instructions.
For trap code it is important that the assembler not naively clobber
this register until it has been saved; a special assembler mode is
required for this.

\subsubsection*{\textit{spill} (1)} (synthesized)

Spill some registers to make room to work.
Because this is a system call handler, and system calls (being calls)
can destroy caller-save registers, saving those is not technically
necessary but the original Barrelfish code does so anyway, and we
follow that precedent, partly to demonstrate that we can also
successfully synthesize other trap handlers where there is no such
leeway.

The number of registers that must be spilled.
The code needed to locate the register save area has up to three
simultaneous live values, so in principle three registers must be
spilled, but on MIPS there are two registers reserved for scratch use
during trap handling so the number can be cut down to one
The method for locating the spill area depends on the machine as
well.

\subsubsection*{\textit{check-kern} (2)} (synthesized)

Check whether the trap came from kernel or user mode, and branch
accordingly.
This information is found in some field of some control register on
most machines.

\subsubsection*{\textit{load-got} (3)} (synthesized)

Load the global offset table base address.
As we mentioned in \autoref{sec:overview}, the Barrelfish kernel is
build as position-independent code, and even though it is not linked
witih shared libraries, on some machines a plain position-independent
data access requires the use of the global offset table.
(RISC-V and x86\_64 have PC-relative addressing that avoids the need
unless a shared library is involved; but on ARM the small immediate
fields in instructions mean that direct PC-relative addressing does
not have enough range.
Meanwhile MIPS does not have PC-relative data addressing at all in the
versions we target.)

The original Barrelfish code keeps the global offset table base in a
control register that ARM provides for arbitrary kernel use, rather
than assuming a fixed offset from the code segment.
For MIPS we carry over this behavior by assuming the existence of a
per-CPU wired page mapping at a fixed address.
This page holds the global offset table base, as well as the spill
space used by the spill block.
For RISC-V and x86\_64 we assume that ordinary PC-relative addressing
is sufficient, as anything else requires substantial changes to
Barrelfish and likely also the C compiler and is beyond the scope of
this work.

\subsubsection*{\textit{get-disp} (4)} (synthesized)

Load the address of the current dispatcher.
The Barrelfish ``dispatcher'' is effectively the process structure;
it is pointed to by a thing called a dispatcher control block, and
the current dispatcher control block is kept in a global variable.
The global variable must be accessed with a PIC reference, so this
block must specify that the PIC register has been loaded (if
necessary) as part of its precondition.

We model PIC accesses in \casp by tagging assembler labels with their
required access type (absolute, PC-relative, or shared library).
Then we define a single family of operations (instructions) that refer
to assembler labels, and within the definitions of those operations
control the exact instructions that are issued based on the access
type of the target label.
This avoids unnecessarily exposing the workings of PIC accesses to the
synthesis engine, and avoids needing to model the workings of the
global offset table directly.
(We only model its existence.)

This model has a downside, however: it bakes in the identity of the
PIC register, which is fine for ordinary code but a headache for trap
code.
For MIPS and ARM we had to make sure that one of the registers spilled
by the spill block is the PIC register so that it can be used by this
block and the previous one.

\subsubsection*{\textit{check-disabled} (5)} (synthesized)

Barrelfish does not save trap context on the kernel stack; instead,
the Barrelfish dispatcher has two register save areas, one for use
when the dispatcher is ``enabled'' (running ordinary user code) and
one for when it is ``disabled'' (running certain system code related
to IPC and scheduling).
The trap code needs to pick which save area to use, and to do that it
uses two criteria: either (a) the ``disabled'' flag (a field in the
dispatcher structure) is set, or (b) the trap PC is within a critical
region whose bounds are kept in the dispatcher structure.
This block checks the first criterion; if the disabled flag is set, it
branches to the set-disabled block.

\subsubsection*{\textit{findpc} (6)} (synthesized)

Load the program counter from the trap into a general purpose register.
This does nothing on ARMv7 (the trap PC is left by the hardware in a
general-purpose register already) 

\subsubsection*{\textit{check-low} (7)} (synthesized)

Check the trap PC against the low bound of the critical region, and 
if below it branch to the set-enabled block.

\subsubsection*{\textit{check-high} (8)} (synthesized)

Check the trap PC against the high bound of the critical region, and 
if below it branch to the set-disabled block.

\subsubsection*{\textit{set-enabled} (9)} (synthesized)

Load the address of the ``enabled'' save area, and branch to the
save-context block.
This block also loads the constant 0 into another register to remember
that the dispatcher is not disabled.

\subsubsection*{\textit{set-disabled} (10)} (synthesized)

Load the address of the ``disabled'' save area, and branch to the
save-context block.
This block also loads the constant 1 into another register to remember
that the dispatcher is disabled.

The original Barrelfish code for ARM had less branching and one joint
block where we now have this block and the previous one, using the ARM
conditional execution features to load either one or the other save
area.
We restructured the code because we found that a more conventional
branching structure produced smaller and more natural code on other
machines, and also because we found that it synthesized noticeably
faster, even for ARM.

\subsubsection*{\textit{save-context}} (handwritten)

Save all the registers into the chosen dispatcher save area.
The ARM version of this is taken from the original Barrelfish code and
adjusted to match the registers we spill in the spill block, which are
not the same as the original due to the need to handle the PIC
register.
The other versions were handwritten.

We do not verify this block (unlike the context saves in the OS/161
examples) because as written the ARM version saves the floating-point
registers, which we do not model.
(Most kernels make use of hardware features to avoid saving the
floating point registers until and unless necessary, but apparently
Barrelfish does not.)
It also uses a special instruction to deal with an ARM-specific
peculiarity of register addressing in trap code, which we also do not
model.
We could have rearranged the structure of the handler to avoid the
need for this instruction but felt that the purposes of our evaluation
were better served by not doing that.

\subsubsection*{\textit{enter-sys}} (handwritten)

This is an ARM-specific block to switch processor modes before
executing ordinary kernel code.
ARM has (multiple) special processor modes for trap handler code, and
one needs to switch out of them before jumping into C code.
We could synthesize this block by adding the necessary instruction and
its associated machine state to our ARMv7 model, but this did not seem
worthwhile.

\subsubsection*{\textit{reshuffle} (11)} (synthesized)

Now that registers have been saved, but before we load the kernel
stack or reload the PIC register, shuffle values around as needed to
avoid clobbering anything.
In particular, on MIPS we avoided spilling more than one register by
using the PIC register as one of the work registers before the
save-context block; but we need the value in it and need to move it
somewhere else before reloading the PIC register.

\subsubsection*{\textit{load-got-2}} (synthesized)

Reload the PIC register with the global offset table base again,
since to avoid using more registers than necessary we overwrote the
result from the previous time.
This block the identical to load-got, so we do not count it again.

\subsubsection*{\textit{initstack} (12)} (synthesized)

Load the stack pointer to point to the kernel stack.
The kernel stack is a global variable, so needs to be accessed with a
PIC data reference.
This is the example used in \autoref{sec:overview}.

\subsubsection*{\textit{moveargs} (13)} (synthesized)

Move the arguments into place for calling the C-level system call
handler.
This does not need to do anything except on MIPS, since on the other
machines we pick the work registers spilled and used before
save-context to be the argument registers.
On MIPS this block moves values from the trap scratch registers to the
argument registers.
On MIPS it also makes room on the stack for a call frame, since due to
pecularities of MIPS there is a 16-byte space on the stack that the
caller provides to the callee to scribble in.
Because of the latter (and because there are architectures where
arguments need to be placed on the stack, even though we do not target
any of them in this paper) this block must come after initstack.

\subsubsection*{\textit{user-dispatch}} (handwritten)

Jump instruction for tail-call to the C-level system call
handler.
This is a PIC jump so on some platforms it uses the global offset
table and is actually more than one instruction.
The trap return code is elsewhere.

\subsubsection*{\textit{kernel-dispatch}} (handwritten)

Similarly, jump instruction for tail-call to the C-level system call
handler for syscalls that come from the kernel.
The trap return code is elsewhere.

On ARM the path that leads to this block jumps into C code without
switching out of trap handling mode and without saving registers that
it probably should.
This is technically a bug, but since the handler for system calls that
come from the kernel does nothing but panic, it does not matter.
We have preserved similar behavior for other platforms.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{\textbf{setjmp} (SJ), \textbf{longjmp} (LJ)}

For these there is little to add to the description in
\autoref{sec:usecases}.
In both cases the complete procedure is the two blocks described there
followed by a return instruction.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{\textbf{crt0} (CRT)}

\texttt{crt0}, the user-level startup code, has nine blocks total, the
extra two being call instructions:

\subsubsection*{\textit{initstack} (1)} (synthesized)

This block aligns the stack pointer, and on MIPS also makes room for a
call frame.
In OS/161, to simplify the lives of students writing the code to place
argument strings on the stacks of new processes, the user startup code 
assumes that the stack pointer given on entry might not be adequately
aligned and attends to that itself.

\subsubsection*{\textit{savevals} (2)} (synthesized)

This block saves the kernel-passed values of \texttt{argv} and
\texttt{environ} into private global variables used by libc.
Because OS/161 does not support shared libraries, they do not need to
be PIC references.
If it did, adjusting the specification would be trivial but the
procedure would also need an additional block to load the PIC
register.

\subsubsection*{\textit{initregs} (3)} (synthesized)

This block initializes the global pointer register on MIPS and RISC-V
using a symbol provided by the linker.
It can also be leveraged to do any other machine-specific
initializations that might be required.

\subsubsection*{\textit{mainargplace} (4)} (synthesized)

This moves the arguments into place for calling \texttt{main}.
This block is actually empty for all our target machines, because the
registers the kernel uses to pass the arguments are the same as the
registers used for arguments by the standard function call ABI.
This is not necessarily the case, however, and furthermore on machines
where the arguments go on the stack this block would be needed to put
them there.
(Placing them on the stack from the kernel is possible, but not
desirable, especially for automatic porting, as the kernel is set up
to assume they are passed in registers.)

\subsubsection*{\textit{maincall}} (handwritten)

Call instruction for calling \texttt{main}.

\subsubsection*{\textit{exitsave} (5)} (synthesized)

This block moves the return value from \texttt{main} into a
callee-save register, so it will not be destroyed by the call to
\texttt{exit}.
As mentioned in \autoref{sec:usecases}, this code is written to
assume that \texttt{exit} might return, even though normally it does
not.
The implementation of \texttt{exit} is student-written, which means
both that it might not work as intended and also that it does not
exist in the baseline version of OS/161 given to students.
In the latter case, it does in fact return (with an error indicating
that there is no such system call) and something needs to be done in
this case; the choice was to loop forever calling \texttt{exit}
repeatedly.

\subsubsection*{\texttt{exitargplace} (6)} (synthesized)

Place the argument to \texttt{exit}.
This moves it from the callee-save register the previous block placed
it in.
Because this block is a branch target, the value in the return value
register from the call to \texttt{main} may not be valid.

\subsubsection*{\textit{exitcall}} (handwritten)

Call instruction for calling \texttt{exit}.

\subsubsection*{\texttt{loop} (7)} (synthesized)

Unconditional branch back to the exitargplace block.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{\textit{syscallstub (SYS)}}

The user-level system call stubs in OS/161 are split into two parts;
one is repeated for each system call and one is shared by all the
system calls.
There are six blocks total, the first three being per-call and the
last three being shared:

\subsubsection*{\textit{loadnum} (1)} (synthesized)

Load the system call number into the register used by the system call
ABI for that purpose.
On ARM system call numbers are placed in the instruction as immediates
instead, so this block is empty.

\subsubsection*{\textit{trapwithnum}} (handwritten)

Single instruction to issue the system call, on machines where it 
contains the call number (ARM).

\subsubsection*{\textit{jump} (2)} (synthesized)

Unconditional jump to the shared code.

\subsubsection*{\textit{trapnonum}} (handwritten)

Single instruction to issue the system call, on machines where it does
not contain the call number (MIPS, RISC-V, x86\_64).

\subsubsection*{\textit{seterrno} (3)} (synthesized)

Convert from the machine-level system call ABI to the C function call
ABI.
Since time immemorial the system call return value ABI on Unix-like
systems has been that there is one result register in which the
kernel returns a value.
This value is either the return value (if the call succeeded), or an
error code (if the call failed), and the state of the carry flag
reports whether the call failed: if set, the call failed.
Historically on some systems some calls return two values in two
registers, or sometimes in halves of one register; OS/161 does not do
this.
Calls that return double-width values (e.g. 64-bit values on 32-bit
platforms, such as \texttt{lseek}) use two registers.
And on machines with no carry flag, such as MIPS and now also RISC-V,
one of the argument registers is used to hold the success or failure
code.

Conversely, the C function call ABI does not have a failure flag, so
the interface for system calls has long been that on success, the
return value is returned, and on failure, -1 is returned (in both
registers for double-wide values) and the error code is placed in the
global (or per-thread) variable \texttt{errno}.

Our specification abstracts over all this for all the machines.

\subsubsection*{\textit{ret}} (handwritten)

A return instruction.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{\textit{cpu-irqoff (IRQ)}}

There is nothing to add to the description in \autoref{sec:usecases}
besides the by-now predictable addendum that the block that does the
work is followed by a handwritten block containing a return
instruction.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{\textit{thread-switch (TS)}}

This consists of seven blocks, only one (the return instruction)
handwritten.

\subsubsection*{\textit{entry} (1)} (synthesized)

This block makes space on the stack to save registers.
The model in OS/161 is that callee-save registers are pushed on the
stack, and the stack pointer is saved in the thread structure; the
arguments to the procedure are pointers to the stack pointer slots in
the old and new thread structures respectively.

\subsubsection*{\textit{saveregs} (2)} (verification only)

This saves the callee-save registers (and return address register, on
machines that have one) to the stack. 

On machines where the current thread pointer is kept in a register
that is ordinarily callee-save (a high-level porting decision beyond
the direct scope of this paper), that register needs to be left off
the list of registers to save, because doing so interacts badly with
the \MI code that manages the current thread pointer.

\subsubsection*{\textit{savestack} (3)} (synthesized)

This block writes the stack pointer through the first argument to the
stack pointer slot of the old thread.

\subsubsection*{\textit{loadstack} (4)} (synthesized)

This block reads the stack pointer via the second argument from the
stack pointer slot of the new thread.

\subsubsection*{\textit{loadregs} (5)} (verification only)

This loads the callee-save registers from the stack.

\subsubsection*{\textit{cleanup} (6)} (synthesized)

This clears the stack frame for return.

\subsubsection*{\textit{ret}} (handwritten)

This block contains a return instruction.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% and some comparative analysis of the OS/161 and bfish trap handlers
% would be nice if we had the OS/161 trap handler in this paper :-(

